liquidSVM: A Fast and Versatile SVM package

liquidSVM is a package written in C++ that provides SVM-type solvers for various classification and regression tasks. Because of a fully integrated hyper-parameter selection, very carefully implemented solvers, multi-threading and GPU support, and several built-in data decomposition strategies it provides unprecedented speed for small training sizes as well as for data sets of tens of millions of samples. Besides the C++ API and a command line interface, bindings to R, MATLAB, Java, Python, and Spark are available. We present a brief description of the package and report experimental comparisons to other SVM packages.

==> benchmarks/tables/combinedLarge-1000.tex <==
\begin{table}[htp]
\centering
\begingroup\footnotesize
\scalebox{0.7}{
\begin{tabular}{lrr|rrrrrr|rrrrr}
  \toprule
 & \texttt{size} & \texttt{dim} & \texttt{liquidSVM} & \texttt{(sec.)} & \texttt{(libsvm grid)} & \texttt{Overlap} & \texttt{Bsvm} & \texttt{Esvm} & \texttt{liquidSVM} & \texttt{(libsvm grid)} & \texttt{Overlap} & \texttt{Bsvm} & \texttt{Esvm} \\ 
  \midrule
\textsc{covtype} & 10000 & 54 & $\times 1.0 $ & 11.7s & $\times 0.7 $ & $\times 2.4 $ & $\times 521.8 $ & $\times 40.2 $ & 16.67 & 17.03 & 16.60 & 19.90 & 21.86 \\ 
  \textsc{covtype} & 40000 & 54 & $\times 1.0 $ & 50.2s & $\times 0.7 $ & $\times 5.9 $ & $\times 445.8 $ & $\times 49.3 $ & 10.80 & 13.23 & 10.29 & 19.34 & 19.80 \\ 
  \textsc{covtype} & 100000 & 54 & $\times 1.0 $ & 117.6s & $\times 0.7 $ & $\times 8.4 $ & $\times 430.0 $ & $\times 87.8 $ & 7.97 & 10.91 & 7.09 & 18.41 & 19.12 \\ 
  \textsc{ijcnn1} & 49990 & 23 & $\times 1.0 $ & 39.1s & $\times 1.0 $ & $\times 8.1 $ & $\times 549.2 $ & $\times 49.6 $ & 1.91 & 1.65 & 1.16 & 1.62 & 6.45 \\ 
  \textsc{webspam} & 280000 & 255 & $\times 1.0 $ & 374.5s & $\times 1.0 $ & $\times 91.8 $ & $\times 407.8 $ & $\times 474.5 $ & 1.63 & 1.80 & 0.93 & 2.61 & 4.11 \\ 
   \bottomrule
\end{tabular}
}
\endgroup
\caption{Relative training time for different implementations in the left part and classification error in the right part (k=1000).} 
\label{table:combinedLarge-1000}
\end{table}


==> benchmarks/tables/combinedLarge-3000.tex <==
\begin{table}[htp]
\centering
\begingroup\footnotesize
\scalebox{0.7}{
\begin{tabular}{lrr|rrrrrr|rrrrr}
  \toprule
 & \texttt{size} & \texttt{dim} & \texttt{liquidSVM} & \texttt{(sec.)} & \texttt{(libsvm grid)} & \texttt{Overlap} & \texttt{Bsvm} & \texttt{Esvm} & \texttt{liquidSVM} & \texttt{(libsvm grid)} & \texttt{Overlap} & \texttt{Bsvm} & \texttt{Esvm} \\ 
  \midrule
\textsc{covtype} & 10000 & 54 & $\times 1.0 $ & 23.9s & $\times 0.8 $ & $\times 2.0 $ & $\times 1736.0 $ & $\times 863.5 $ & 16.58 & 16.46 & 16.31 & 17.10 & 17.31 \\ 
  \textsc{covtype} & 40000 & 54 & $\times 1.0 $ & 99.7s & $\times 0.8 $ & $\times 3.1 $ & $\times 1030.1 $ & $\times 233.7 $ & 10.76 & 12.82 & 10.60 & 15.66 & 16.22 \\ 
  \textsc{covtype} & 100000 & 54 & $\times 1.0 $ & 251s & $\times 0.8 $ & $\times 7.1 $ & $\times 839.8 $ & $\times 124.0 $ & 7.72 & 10.74 & 7.30 & 14.72 & 15.71 \\ 
  \textsc{ijcnn1} & 49990 & 23 & $\times 1.0 $ & 95.5s & $\times 1.1 $ & $\times 1.7 $ & $\times 1157.4 $ & $\times 119.5 $ & 1.34 & 1.11 & 1.38 & 1.12 & 3.64 \\ 
  \textsc{webspam} & 280000 & 255 & $\times 1.0 $ & 758.8s & $\times 1.0 $ & $\times 199.2 $ & $\times 980.0 $ & $\times 241.4 $ & 1.35 & 1.48 & 0.84 & 2.23 & 3.06 \\ 
   \bottomrule
\end{tabular}
}
\endgroup
\caption{Relative training time for different implementations in the left part and classification error in the right part (k=3000).} 
\label{table:combinedLarge-3000}
\end{table}


==> benchmarks/tables/combinedLarge-500.tex <==
\begin{table}[htp]
\centering
\begingroup\footnotesize
\scalebox{0.7}{
\begin{tabular}{lrr|rrrrrr|rrrrr}
  \toprule
 & \texttt{size} & \texttt{dim} & \texttt{liquidSVM} & \texttt{(sec.)} & \texttt{(libsvm grid)} & \texttt{Overlap} & \texttt{Bsvm} & \texttt{Esvm} & \texttt{liquidSVM} & \texttt{(libsvm grid)} & \texttt{Overlap} & \texttt{Bsvm} & \texttt{Esvm} \\ 
  \midrule
\textsc{covtype} & 10000 & 54 & $\times 1.0 $ & 8s & $\times 0.7 $ & $\times 3.7 $ & $\times 252.1 $ & $\times 130.4 $ & 16.78 & 17.04 & 15.84 & 21.96 & 22.43 \\ 
  \textsc{covtype} & 40000 & 54 & $\times 1.0 $ & 34.2s & $\times 0.7 $ & $\times 7.2 $ & $\times 242.5 $ & $\times 66.2 $ & 11.52 & 13.78 & 10.19 & 20.89 & 21.93 \\ 
  \textsc{covtype} & 100000 & 54 & $\times 1.0 $ & 81.8s & $\times 0.7 $ & $\times 8.6 $ & $\times 223.8 $ & $\times 69.0 $ & 8.27 & 11.12 & 7.22 & 21.08 & 21.65 \\ 
  \textsc{ijcnn1} & 49990 & 23 & $\times 1.0 $ & 26.7s & $\times 1.0 $ & $\times 22.3 $ & $\times 314.5 $ & $\times 62.2 $ & 2.82 & 2.10 & 1.21 & 2.17 & 6.96 \\ 
  \textsc{webspam} & 280000 & 255 & $\times 1.0 $ & 282.5s & $\times 1.0 $ & $\times 62.3 $ & $\times 211.8 $ & $\times 164.7 $ & 1.77 & 1.93 & 0.97 & 3.04 & 5.48 \\ 
   \bottomrule
\end{tabular}
}
\endgroup
\caption{Relative training time for different implementations in the left part and classification error in the right part (k=500).} 
\label{table:combinedLarge-500}
\end{table}


==> benchmarks/tables/errLarge.tex <==
\begingroup\footnotesize
\scalebox{0.8}{
\begin{tabular}{lrrrrr}
  \toprule
 & \texttt{liquidSVM} & \texttt{(libsvm grid)} & \texttt{Overlap} & \texttt{Bsvm} & \texttt{Esvm} \\ 
  \midrule
\textsc{covtype.10000} & 16.58 & 16.46 & 16.31 & 17.10 & 17.31 \\ 
  \textsc{covtype.40000} & 10.76 & 12.82 & 10.60 & 15.66 & 16.22 \\ 
  \textsc{covtype.100000} & 7.72 & 10.74 & 7.30 & 14.72 & 15.71 \\ 
  \textsc{ijcnn1} & 1.34 & 1.11 & 1.38 & 1.12 & 3.64 \\ 
  \textsc{webspam} & 1.35 & 1.48 & 0.84 & 2.23 & 3.06 \\ 
   \bottomrule
\end{tabular}
}
\endgroup


==> benchmarks/tables/errOur.tex <==
\begin{table}[htp]
\centering
\begingroup\footnotesize
\scalebox{0.8}{
\begin{tabular}{lrrrr}
  \toprule
 & \textsc{bank-marketing} & \textsc{cod-rna} & \textsc{covtype} & \textsc{thyroid-ann} \\ 
  \midrule
threads=1 & 10.55 & 4.00 & 18.86 &  \\ 
  threads=2 & 10.61 & 3.97 & 18.85 &  \\ 
  threads=3 & 10.58 & 3.98 & 18.75 &  \\ 
  threads=4 & 10.54 & 3.98 & 18.57 &  \\ 
  grid\_choice=1 & 10.56 & 4.03 & 18.75 &  \\ 
  grid\_choice=2 & 10.66 & 4.00 & 18.63 &  \\ 
  adaptivity\_control=1 & 10.57 & 4.00 & 18.80 &  \\ 
  adaptivity\_control=2 & 10.55 & 3.99 & 18.77 &  \\ 
  adaptivity\_control=2, grid\_choice=2 & 10.59 & 4.01 & 18.73 &  \\ 
  voronoi=5 & 10.69 & 3.95 & 18.84 &  \\ 
  voronoi=6 & 10.80 & 3.98 & 18.91 &  \\ 
  voronoi=c(5,1000) & 10.79 & 3.94 & 18.94 &  \\ 
  voronoi=c(6,1000) & 10.96 & 4.09 & 19.29 &  \\ 
   \bottomrule
\end{tabular}
}
\endgroup
\caption{Relative mean classification errors for different configurations (n=6000, arch=native).} 
\label{table:errOur}
\end{table}


==> benchmarks/tables/timeOur-1000-archs.tex <==
\begin{table}[htp]
\centering
\begingroup\footnotesize
\scalebox{0.8}{
\begin{tabular}{l|rrr|rrr|rrr|rrr}
  \toprule
 & \begin{sideways} \textsc{bank-marketing} \end{sideways} & \begin{sideways} \textsc{bank-marketing} \end{sideways} & \begin{sideways} \textsc{bank-marketing} \end{sideways} & \begin{sideways} \textsc{cod-rna} \end{sideways} & \begin{sideways} \textsc{cod-rna} \end{sideways} & \begin{sideways} \textsc{cod-rna} \end{sideways} & \begin{sideways} \textsc{covtype} \end{sideways} & \begin{sideways} \textsc{covtype} \end{sideways} & \begin{sideways} \textsc{covtype} \end{sideways} & \begin{sideways} \textsc{thyroid-ann} \end{sideways} & \begin{sideways} \textsc{thyroid-ann} \end{sideways} & \begin{sideways} \textsc{thyroid-ann} \end{sideways} \\ 
  \midrule
\texttt{threads=1} & 0.90 & 0.80 & 0.79 & 0.75 & 0.71 & 0.70 & 1.03 & 0.91 & 0.89 & 0.95 & 0.88 & 0.86 \\ 
  \texttt{threads=2} & 0.86 & 0.80 & 0.77 & 0.74 & 0.69 & 0.68 & 1.01 & 0.88 & 0.87 & 0.94 & 0.86 & 0.84 \\ 
  \texttt{threads=3} & 0.82 & 0.71 & 0.71 & 0.69 & 0.62 & 0.60 & 0.94 & 0.80 & 0.78 & 0.91 & 0.78 & 0.76 \\ 
  \texttt{threads=4} & 0.80 & 0.68 & 0.67 & 0.66 & 0.58 & 0.57 & 0.89 & 0.76 & 0.75 & 0.86 & 0.74 & 0.72 \\ 
  \texttt{grid\_choice=1} & 1.98 & 1.64 & 1.58 & 1.46 & 1.23 & 1.22 & 2.39 & 1.90 & 1.82 & 2.36 & 1.83 & 1.81 \\ 
  \texttt{grid\_choice=2} & 6.73 & 4.77 & 4.69 & 4.42 & 3.08 & 3.19 & 8.03 & 5.86 & 5.59 & 8.39 & 5.69 & 5.95 \\ 
  \texttt{adaptivity\_control=1} & 0.70 & 0.60 & 0.60 & 0.57 & 0.50 & 0.50 & 0.77 & 0.64 & 0.64 & 0.72 & 0.58 & 0.60 \\ 
  \texttt{adaptivity\_control=2} & 0.60 & 0.53 & 0.52 & 0.50 & 0.42 & 0.44 & 0.68 & 0.57 & 0.59 & 0.65 & 0.55 & 0.53 \\ 
  \texttt{adaptivity\_control=2, grid\_choice=2} & 3.22 & 2.42 & 2.37 & 2.11 & 1.46 & 1.51 & 3.27 & 2.77 & 2.21 & 3.55 & 2.54 & 2.59 \\ 
  \texttt{voronoi=5} & 0.80 & 0.68 & 0.66 & 0.65 & 0.57 & 0.56 & 0.88 & 0.76 & 0.75 & 0.85 & 0.74 & 0.72 \\ 
  \texttt{voronoi=6} & 0.79 & 0.68 & 0.66 & 0.64 & 0.58 & 0.57 & 0.89 & 0.77 & 0.74 & 0.85 & 0.73 & 0.72 \\ 
  \texttt{voronoi=c(5,1000)} & 0.78 & 0.69 & 0.66 & 0.65 & 0.58 & 0.56 & 0.89 & 0.76 & 0.74 & 0.83 & 0.75 & 0.72 \\ 
  \texttt{voronoi=c(6,1000)} & 0.78 & 0.68 & 0.67 & 0.65 & 0.58 & 0.57 & 0.89 & 0.76 & 0.75 & 0.83 & 0.73 & 0.71 \\ 
   \bottomrule
\end{tabular}
}
\endgroup
\caption{Training times (in sec.) for different compile architectures: from left to right they are
                                           \texttt{SSE2}, \texttt{AVX}, and \texttt{AVX2}, averaged over 10 repetitions with n=1000.} 
\label{table:timeOur-1000-archs}
\end{table}


==> benchmarks/tables/timeOur-2000-archs.tex <==
\begin{table}[htp]
\centering
\begingroup\footnotesize
\scalebox{0.8}{
\begin{tabular}{l|rrr|rrr|rrr|rrr}
  \toprule
 & \begin{sideways} \textsc{bank-marketing} \end{sideways} & \begin{sideways} \textsc{bank-marketing} \end{sideways} & \begin{sideways} \textsc{bank-marketing} \end{sideways} & \begin{sideways} \textsc{cod-rna} \end{sideways} & \begin{sideways} \textsc{cod-rna} \end{sideways} & \begin{sideways} \textsc{cod-rna} \end{sideways} & \begin{sideways} \textsc{covtype} \end{sideways} & \begin{sideways} \textsc{covtype} \end{sideways} & \begin{sideways} \textsc{covtype} \end{sideways} & \begin{sideways} \textsc{thyroid-ann} \end{sideways} & \begin{sideways} \textsc{thyroid-ann} \end{sideways} & \begin{sideways} \textsc{thyroid-ann} \end{sideways} \\ 
  \midrule
\texttt{threads=1} & 3.27 & 2.93 & 2.88 & 2.76 & 2.57 & 2.53 & 3.94 & 3.40 & 3.33 & 3.43 & 3.02 & 2.97 \\ 
  \texttt{threads=2} & 2.59 & 2.24 & 2.16 & 2.05 & 1.86 & 1.81 & 3.08 & 2.60 & 2.54 & 2.66 & 2.30 & 2.27 \\ 
  \texttt{threads=3} & 2.38 & 1.94 & 1.87 & 1.80 & 1.56 & 1.54 & 2.83 & 2.32 & 2.24 & 2.37 & 1.99 & 1.92 \\ 
  \texttt{threads=4} & 2.22 & 1.80 & 1.73 & 1.65 & 1.43 & 1.40 & 2.73 & 2.17 & 2.10 & 2.30 & 1.82 & 1.81 \\ 
  \texttt{grid\_choice=1} & 6.25 & 4.79 & 4.59 & 3.96 & 3.12 & 3.01 & 8.52 & 6.17 & 5.88 & 7.39 & 5.19 & 4.91 \\ 
  \texttt{grid\_choice=2} & 26.62 & 17.29 & 16.50 & 14.26 & 9.80 & 9.44 & 34.18 & 22.27 & 21.72 & 34.84 & 23.01 & 21.19 \\ 
  \texttt{adaptivity\_control=1} & 1.89 & 1.55 & 1.56 & 1.39 & 1.24 & 1.21 & 2.40 & 1.92 & 1.88 & 1.73 & 1.44 & 1.38 \\ 
  \texttt{adaptivity\_control=2} & 1.69 & 1.31 & 1.31 & 1.23 & 1.09 & 1.07 & 2.16 & 1.68 & 1.64 & 1.49 & 1.16 & 1.19 \\ 
  \texttt{adaptivity\_control=2, grid\_choice=2} & 10.08 & 8.04 & 7.40 & 5.35 & 4.59 & 3.96 & 12.53 & 7.97 & 7.92 & 9.49 & 6.62 & 6.97 \\ 
  \texttt{voronoi=5} & 2.20 & 1.77 & 1.73 & 1.66 & 1.43 & 1.41 & 2.73 & 2.17 & 2.08 & 2.23 & 1.84 & 1.76 \\ 
  \texttt{voronoi=6} & 2.21 & 1.81 & 1.76 & 1.65 & 1.43 & 1.41 & 2.75 & 2.17 & 2.12 & 2.22 & 1.80 & 1.73 \\ 
  \texttt{voronoi=c(5,1000)} & 1.81 & 1.54 & 1.54 & 1.59 & 1.57 & 1.67 & 2.12 & 1.81 & 1.77 & 2.02 & 1.72 & 1.69 \\ 
  \texttt{voronoi=c(6,1000)} & 1.40 & 1.27 & 1.22 & 1.17 & 1.10 & 1.05 & 1.66 & 1.41 & 1.39 & 1.38 & 1.22 & 1.17 \\ 
   \bottomrule
\end{tabular}
}
\endgroup
\caption{Training times (in sec.) for different compile architectures: from left to right they are
                                           \texttt{SSE2}, \texttt{AVX}, and \texttt{AVX2}, averaged over 10 repetitions with n=2000.} 
\label{table:timeOur-2000-archs}
\end{table}


==> benchmarks/tables/timeOur-4000-archs.tex <==
\begin{table}[htp]
\centering
\begingroup\footnotesize
\scalebox{0.8}{
\begin{tabular}{l|rrr|rrr|rrr|rrr}
  \toprule
 & \begin{sideways} \textsc{bank-marketing} \end{sideways} & \begin{sideways} \textsc{bank-marketing} \end{sideways} & \begin{sideways} \textsc{bank-marketing} \end{sideways} & \begin{sideways} \textsc{cod-rna} \end{sideways} & \begin{sideways} \textsc{cod-rna} \end{sideways} & \begin{sideways} \textsc{cod-rna} \end{sideways} & \begin{sideways} \textsc{covtype} \end{sideways} & \begin{sideways} \textsc{covtype} \end{sideways} & \begin{sideways} \textsc{covtype} \end{sideways} & \begin{sideways} \textsc{thyroid-ann} \end{sideways} & \begin{sideways} \textsc{thyroid-ann} \end{sideways} & \begin{sideways} \textsc{thyroid-ann} \end{sideways} \\ 
  \midrule
\texttt{threads=1} & 12.55 & 11.34 & 11.10 & 10.51 & 9.85 & 9.71 & 15.41 & 13.35 & 12.99 & 13.11 & 11.70 & 11.36 \\ 
  \texttt{threads=2} & 9.12 & 7.80 & 7.55 & 7.01 & 6.35 & 6.11 & 11.60 & 9.52 & 9.21 & 9.21 & 7.96 & 7.74 \\ 
  \texttt{threads=3} & 8.29 & 6.78 & 6.64 & 6.10 & 5.36 & 5.28 & 10.68 & 8.47 & 8.19 & 8.37 & 6.92 & 6.71 \\ 
  \texttt{threads=4} & 7.98 & 6.44 & 6.31 & 5.78 & 4.99 & 4.88 & 10.43 & 8.10 & 7.76 & 8.16 & 6.49 & 6.26 \\ 
  \texttt{grid\_choice=1} & 25.30 & 17.93 & 17.32 & 14.10 & 10.86 & 10.38 & 34.80 & 24.00 & 23.43 & 29.47 & 19.70 & 18.85 \\ 
  \texttt{grid\_choice=2} & 112.65 & 73.27 & 70.09 & 52.64 & 36.40 & 35.28 & 152.60 & 100.76 & 96.10 & 159.31 & 98.05 & 94.10 \\ 
  \texttt{adaptivity\_control=1} & 6.82 & 5.73 & 5.52 & 4.96 & 4.28 & 4.37 & 9.18 & 7.34 & 6.90 & 5.67 & 4.69 & 4.52 \\ 
  \texttt{adaptivity\_control=2} & 5.59 & 4.82 & 4.61 & 4.15 & 3.95 & 3.66 & 8.44 & 6.30 & 6.14 & 4.75 & 4.14 & 3.74 \\ 
  \texttt{adaptivity\_control=2, grid\_choice=2} & 38.92 & 28.29 & 25.72 & 18.85 & 14.05 & 13.02 & 46.64 & 24.79 & 26.79 & 26.80 & 19.64 & 18.27 \\ 
  \texttt{voronoi=5} & 5.33 & 4.35 & 4.45 & 4.54 & 4.62 & 4.37 & 7.34 & 5.32 & 5.71 & 5.99 & 4.97 & 4.74 \\ 
  \texttt{voronoi=6} & 3.60 & 2.96 & 2.86 & 2.84 & 2.53 & 2.44 & 4.88 & 3.92 & 3.78 & 3.53 & 2.90 & 2.74 \\ 
  \texttt{voronoi=c(5,1000)} & 4.88 & 4.18 & 4.15 & 4.22 & 3.83 & 3.60 & 5.35 & 4.11 & 4.10 & 6.44 & 5.12 & 5.32 \\ 
  \texttt{voronoi=c(6,1000)} & 2.72 & 2.36 & 2.38 & 2.31 & 2.09 & 2.15 & 3.25 & 2.76 & 2.73 & 2.51 & 2.26 & 2.21 \\ 
   \bottomrule
\end{tabular}
}
\endgroup
\caption{Training times (in sec.) for different compile architectures: from left to right they are
                                           \texttt{SSE2}, \texttt{AVX}, and \texttt{AVX2}, averaged over 10 repetitions with n=4000.} 
\label{table:timeOur-4000-archs}
\end{table}


==> benchmarks/tables/timeOur-6000-archs.tex <==
\begin{table}[htp]
\centering
\begingroup\footnotesize
\scalebox{0.8}{
\begin{tabular}{l|rrr|rrr|rrr|rrr}
  \toprule
 & \begin{sideways} \textsc{bank-marketing} \end{sideways} & \begin{sideways} \textsc{bank-marketing} \end{sideways} & \begin{sideways} \textsc{bank-marketing} \end{sideways} & \begin{sideways} \textsc{cod-rna} \end{sideways} & \begin{sideways} \textsc{cod-rna} \end{sideways} & \begin{sideways} \textsc{cod-rna} \end{sideways} & \begin{sideways} \textsc{covtype} \end{sideways} & \begin{sideways} \textsc{covtype} \end{sideways} & \begin{sideways} \textsc{covtype} \end{sideways} & \begin{sideways} \textsc{thyroid-ann} \end{sideways} & \begin{sideways} \textsc{thyroid-ann} \end{sideways} & \begin{sideways} \textsc{thyroid-ann} \end{sideways} \\ 
  \midrule
\texttt{threads=1} & 27.87 & 25.27 & 24.72 & 23.10 & 21.83 & 21.44 & 33.86 & 29.46 & 28.85 &  &  &  \\ 
  \texttt{threads=2} & 19.69 & 16.91 & 16.48 & 14.93 & 13.52 & 13.30 & 24.96 & 20.53 & 19.93 &  &  &  \\ 
  \texttt{threads=3} & 17.89 & 14.89 & 14.67 & 13.21 & 11.65 & 11.48 & 23.09 & 18.42 & 17.90 &  &  &  \\ 
  \texttt{threads=4} & 17.35 & 14.06 & 13.81 & 12.52 & 10.80 & 10.64 & 22.46 & 17.52 & 16.99 &  &  &  \\ 
  \texttt{grid\_choice=1} & 57.15 & 41.01 & 39.40 & 30.85 & 23.84 & 23.25 & 79.98 & 55.21 & 53.80 &  &  &  \\ 
  \texttt{grid\_choice=2} & 266.36 & 176.77 & 168.54 & 121.97 & 82.49 & 79.26 & 376.11 & 241.72 & 234.04 &  &  &  \\ 
  \texttt{adaptivity\_control=1} & 14.67 & 12.41 & 12.11 & 10.95 & 9.64 & 9.69 & 19.78 & 14.99 & 14.71 &  &  &  \\ 
  \texttt{adaptivity\_control=2} & 11.55 & 10.27 & 10.32 & 9.16 & 8.48 & 8.31 & 16.68 & 13.53 & 13.37 &  &  &  \\ 
  \texttt{adaptivity\_control=2, grid\_choice=2} & 91.60 & 58.95 & 58.69 & 36.09 & 28.60 & 27.50 & 65.50 & 50.19 & 47.58 &  &  &  \\ 
  \texttt{voronoi=5} & 9.26 & 7.80 & 7.56 & 7.27 & 7.03 & 6.39 & 13.32 & 9.16 & 8.78 &  &  &  \\ 
  \texttt{voronoi=6} & 5.27 & 4.47 & 4.46 & 4.17 & 3.66 & 3.64 & 6.74 & 5.47 & 5.29 &  &  &  \\ 
  \texttt{voronoi=c(5,1000)} & 8.27 & 6.82 & 6.71 & 7.88 & 6.23 & 6.89 & 9.70 & 8.47 & 8.56 &  &  &  \\ 
  \texttt{voronoi=c(6,1000)} & 3.84 & 3.61 & 3.61 & 3.34 & 2.98 & 2.97 & 4.57 & 4.19 & 4.19 &  &  &  \\ 
   \bottomrule
\end{tabular}
}
\endgroup
\caption{Training times (in sec.) for different compile architectures: from left to right they are
                                           \texttt{SSE2}, \texttt{AVX}, and \texttt{AVX2}, averaged over 10 repetitions with n=6000.} 
\label{table:timeOur-6000-archs}
\end{table}


==> benchmarks/tables/traintimeLarge.tex <==
\begingroup\footnotesize
\scalebox{0.8}{
\begin{tabular}{lrrrrrr}
  \toprule
 & \texttt{liquidSVM} & \texttt{(sec.)} & \texttt{(libsvm grid)} & \texttt{Overlap} & \texttt{Bsvm} & \texttt{Esvm} \\ 
  \midrule
\textsc{covtype.10000} & $\times 1.0 $ & 23.9s & $\times 0.8 $ & $\times 2.0 $ & $\times 1736.0 $ & $\times 863.5 $ \\ 
  \textsc{covtype.40000} & $\times 1.0 $ & 99.7s & $\times 0.8 $ & $\times 3.1 $ & $\times 1030.1 $ & $\times 233.7 $ \\ 
  \textsc{covtype.100000} & $\times 1.0 $ & 251s & $\times 0.8 $ & $\times 7.1 $ & $\times 839.8 $ & $\times 124.0 $ \\ 
  \textsc{ijcnn1} & $\times 1.0 $ & 95.5s & $\times 1.1 $ & $\times 1.7 $ & $\times 1157.4 $ & $\times 119.5 $ \\ 
  \textsc{webspam} & $\times 1.0 $ & 758.8s & $\times 1.0 $ & $\times 199.2 $ & $\times 980.0 $ & $\times 241.4 $ \\ 
   \bottomrule
\end{tabular}
}
\endgroup


==> benchmarks/tables/traintimeOur.tex <==
\begin{table}[htp]
\centering
\begingroup\footnotesize
\scalebox{0.8}{
\begin{tabular}{lrrrr}
  \toprule
 & \begin{sideways} \textsc{bank-marketing} \end{sideways} & \begin{sideways} \textsc{cod-rna} \end{sideways} & \begin{sideways} \textsc{covtype} \end{sideways} & \begin{sideways} \textsc{thyroid-ann} \end{sideways} \\ 
  \midrule
\texttt{threads=1} & 1.79 & 2.01 & 1.70 &  \\ 
  \texttt{threads=2} & 1.19 & 1.25 & 1.17 &  \\ 
  \texttt{threads=3} & 1.06 & 1.08 & 1.05 &  \\ 
  \texttt{threads=4} & 1.00 & 1.00 & 1.00 &  \\ 
  \texttt{grid\_choice=1} & 2.85 & 2.18 & 3.17 &  \\ 
  \texttt{grid\_choice=2} & 12.20 & 7.45 & 13.77 &  \\ 
  \texttt{adaptivity\_control=1} & 0.88 & 0.91 & 0.87 &  \\ 
  \texttt{adaptivity\_control=2} & 0.75 & 0.78 & 0.79 &  \\ 
  \texttt{adaptivity\_control=2, grid\_choice=2} & 4.25 & 2.58 & 2.80 &  \\ 
  \texttt{voronoi=5} & 0.55 & 0.60 & 0.52 &  \\ 
  \texttt{voronoi=6} & 0.32 & 0.34 & 0.31 &  \\ 
  \texttt{voronoi=c(5,1000)} & 0.49 & 0.65 & 0.50 &  \\ 
  \texttt{voronoi=c(6,1000)} & 0.26 & 0.28 & 0.25 &  \\ 
   \bottomrule
\end{tabular}
}
\endgroup
\caption{Training time for different configurations relative to \texttt{thread} and averaged over 10 reptitions (n=6000, arch=native).} 
\label{table:traintimeOur}
\end{table}

